Cheap Recovery: A Key to Self-Managing State

Cluster hash tables (CHTs) are a key persistent-storage component of many large-scale Internet services due to their high performance and scalability. We show that a correctly-designed CHT can also be as easy to manage as a farm of stateless servers. Specifically, we trade away some consistency to obtain reboot-based recovery that is simple, maintains full data availability, and only has modest impact on performance. This simplifies management in two ways. First, it simplifies failure detection by lowering the cost of acting on false positives, allowing us to use simple but aggressive statistical techniques to quickly detect potential failures and node degradations; even when a false alarm is raised or when rebooting will not fix the problem, attempting recovery by rebooting is relatively non-intrusive to system availability and performance. Second, it allows us to re-cast online repartitioning as failure plus recovery, simplifying dynamic scaling and capacity planning. These properties make it possible for the system to be continuously self-adjusting, a key property of self-managing, autonomic systems.

==> abstract.tex <==
Cluster hash tables (CHTs) are a key persistent-storage component of
many large-scale Internet services due to their high performance and
scalability.  We show that a correctly-designed CHT can also be as
easy to manage as a farm of stateless servers.  Specifically, we trade
away some consistency to obtain reboot-based recovery that is simple,
maintains full data availability, and only has modest impact on
performance.  This simplifies management in two ways.  First, it
simplifies failure detection by lowering the cost of acting on false
positives, allowing us to use simple but aggressive statistical
techniques to quickly detect potential failures and node degradations;
even when a false alarm is raised or when rebooting will not fix the
problem, attempting recovery by rebooting is relatively non-intrusive
to system availability and performance.  Second, it allows us to
re-cast online repartitioning as failure plus recovery, simplifying
dynamic scaling and capacity planning.  These properties make it
possible for the system to be continuously self-adjusting, a key
property of self-managing, autonomic systems.


==> conclusion.tex <==
\section{Conclusion}

We combined two techniques---quorums to tolerate replica inconsistency
and single-phase operations to avoid locking---to make reboot-based
recovery fast and non-intrusive in a cluster-based hash table.  One
consequence of this cheap recovery is that we successfully applied
aggressive statistical anomaly-based failure detection to
automatically detect and recover from both fail-stop and fail-stutter
transients.  Furthermore, we used the same recovery mechanism to solve
the distinct problem of incremental scaling without service
interruption.  The net result is a state store that can be managed
with the same types of simple mechanisms and policies as used for
stateless frontends.

Taking a larger view, we believe cheap recovery is an important design
pattern for self-managing systems: when recovery is predictably fast
and has predictably small impact on system availability and
performance, the line between ``normal'' and ``recovery'' operation
becomes blurred.  This makes it acceptable for the system to be
constantly ``recovering,'' a key property of self-managing, autonomic
systems.


==> discussion.tex <==
\section{Discussion and future work}\label{benefits}

In this section, we wrap up the discussion on administration costs and
discuss future work.

\subsection{Reducing administration costs}

Certain kinds of Internet service data, such as billing information,
require the transactional semantics and query generality of a
relational database.  By using a CHT for data that requires durability
but can tolerate our relaxed consistency model and does not need to
support complex queries, one can reduce the size of the relational
database installation, and therefore its administration cost.  The
overhead in setting up and managing the CHT in addition to an existing
database is compensated by the extreme ease of administering the CHT
even at large scale.

\subsection{Future work}

One area of future work involves using cheap recovery to evaluate
different failure detection techniques and parameters.  The low cost
of acting on false positives enables us to replace the manual
parameter-tuning process with one that discovers more optimal
parameters automatically in a similar trial-and-error fashion.  A
second area of future work involves handling permanent disk failures.
With hundreds to thousands of disks, large-scale Internet services
replace disks frequently.  Rather than requiring immediate
replacement, it is important to tolerate a brick being down for
several days or more.  Once the brick is replaced, the system must
automatically integrate the new brick into the system, reconstructing
data from the live bricks as necessary.


==> impl.tex <==
\section{Implementation details}\label{impl}

In this section, we discuss details of the DStore implementation.
Recall that DStore is composed of two components, Dlibs and bricks
shown in Figure \ref{fig:arch}.

A Dlib is a Java class that presents a single-system image with the
consistency model detailed in the previous section.  The Dlib API
exposes {\tt put(key,value)} and {\tt get(key)} methods where keys are
32-bit integers and values are byte arrays.  Dlibs service requests by
issuing read{\slash}write requests to bricks via TCP/IP socket
connections.  In order to act as the {\em coordinator} for these
distributed operations, Dlibs maintain soft state metadata about how
data is partitioned and replicated.  Finally, Dlibs maintain request
latency statistics, which are used in making repartitioning decisions.

Bricks store persistent data accessed via the brick API -- {\tt
write(key,value,ts)}, {\tt read\_val(key)}, and {\tt read\_ts(key)}.
For reading data, {\tt read\_val} returns a value-timestamp pair,
while {\tt read\_ts} returns only the timestamp.  On a {\tt write},
the brick checksums the key-value-timestamp object and writes it
synchronously to disk.  Bricks also cache timestamps in an in-memory
Java Hashtable, and use the file system buffer cache to cache values.
Since the timestamp cache is updated after the value is written to
disk, if a brick fails while processing a write, on a read, it
conservatively returns a timestamp that is no newer than the timestamp
of the value on disk.

Currently, data is stored in files as fixed-length records where the
record size is configured at table-creation time.  Although this
scheme is constrained by its fixed-length nature, it is appropriate
for datasets with low value-size variance, such as Amazon's catalog
metadata database, which has fixed-size entries~\cite{verm:personal}.
Since the underlying storage scheme is orthogonal to DStore's design
techniques and is not critical for evaluating the system's recovery
and manageability, simplicity is the main reason this scheme is used.
Nevertheless, bricks are designed so that it is easy to plug in
different storage schemes.  For example, implementing wrapper code for
Berkeley DB~\cite{bdb} took less than an hour and changing storage
schemes takes a matter of seconds.

Bricks maintain two open TCP/IP socket connections (send and receive)
per Dlib, one control channel used for initiating recovery and
repartitioning, and three message queues (read, put, and ts) serviced
by individual thread pools.  Like router QoS queues, differentiating
requests enables administrators to provision resources and maintain a
minimum level of service for each request type.  Furthermore,
differentiating longer-running write requests from read requests
reduces the service time variance, and subsequently, the average
queuing delay~\cite{trivedi:stats}.

\subsection{Keyspace partitioning}

Storage and throughput capacity is scaled by horizontally partitioning
the hash table across bricks.  Each partition is replicated on a set
of bricks to form a {\em replica group}, the unit upon which quorum
operations are performed.  Keys are partitioned across replica groups
based on the keys' least-significant bits, called the {\em replica
group ID} ({\em RGID}).  Later we show how the keyspace can be
dynamically repartitioned without loss of availability to compensate
for an uneven workload or heterogeneous brick performance.

%  For simplicity we assume an even distribution of keys across the
%  keyspace, though not an even distribution of requests to keys.
%  To achieve even distribution, the keyspace
%  should be split to whatever granularity is required assigning bricks
%  multiple RGID's as necessary; however, since we assume an even
%  distribution of keys, sophisticated partitioning is unnecessary.

Upon startup, each brick is configured with an RGID-mask pair, which
it beacons periodically to distribute metadata and indicate liveness.
For example, if brick $B$ beacons $(1, 11)$, this tells Dlib's to use
the last two bits of the key to find $B$'s RGID, $01$.  Using this
information, Dlibs build a soft-state RGID-to-brick mapping ({\em RGID
map}); to find the replica group storing a given key, Dlibs find the
entry with the longest matching suffix.

The beaconing period is a system-configurable parameter (currently set
to two seconds), so in between beacons, a Dlib's RGID map may become
stale.  Since each brick is the ultimate authority of its own RGID, if
a Dlib sends a request to the wrong brick, the brick returns a {\tt
WRONG\_REPLICA\_GROUP} error.  Once the Dlib's RGID map is updated on
the next beaconing period, the request is sent to the correct set of
bricks.  Finally, a brick can be a part of more than one replica group
by announcing multiple RGIDs.  This feature is used to spread load
across a heterogeneous set of bricks and in the online repartitioning
algorithm described later in this section.

\subsection{Detailed algorithms}

DStore's {\tt put} and {\tt get} algorithms, which were outlined
earlier, are described here in full detail.  For this discussion, let
$N$ be the number of bricks in a replica group, let $WT$ ({\em write
threshold}) be the minimum number of bricks that must reply before a
{\tt put} returns, and let $RT$ ({\em read threshold}) be the minimum
number of bricks that are queried on a {\tt get}.  In DStore, we
choose $WT$ and $RT$ to be a majority -- $\lceil (N+1)/2 \rceil$;
however, in general, $WT$ and $RT$ can be chosen such that the read
and write sets intersect: $WT + RT > N$.\footnote{Quorum systems
generally also require that $2 * WT > N$ so that simultaneous writes
can be ordered; however, we use physical timestamps, which eliminates
this requirement.}

\textbf{Dlib put}: On a {\tt put}, the Dlib generates a physical
timestamp from its local clock and appends its IP address.  The
timestamped value is sent to the entire replica group, but the Dlib
only waits for the first $WT$ responses to ensure the quorum majority
invariant holds, and ignores any subsequent responses.  Pseudocode for
all algorithms are provided in the appendix.

\textbf{Brick write}: When a brick receives a write request, it
overwrites a value only if the new value has a more recent timestamp.
If the new timestamp is older than the current timestamp by
$\Delta_{ts}$, which is set to 1 millisecond, the brick returns {\tt
TIMESTAMP\_ERROR}.

\textbf{Dlib get}: On a {\tt get}, the Dlib selects $RT$ random bricks
from the replica group, and issues a {\tt read\_val} request to one
brick and {\tt read\_ts} requests to the remaining $RT-1$ bricks.
After the value and all the timestamps are returned, the Dlib calls
the {\tt check} method to confirm that the value is up to date.

\textbf{Dlib check}: On each {\tt get}, two checks are performed on
the timestamps.  First, the Dlib checks whether the timestamp for {\tt
value} is the most recent one returned.  If it is, {\tt value} is
returned; otherwise, the value is read from the brick that returned
the most recent timestamp.  Second, the Dlib checks whether at least
$WT$ bricks have the most recent timestamp.  If not, the most recent
value and timestamp are written back to ensure that enough bricks
contain an up-to-date value.  This repair mechanism is used to repair
partial writes arising from Dlib failures.

\subsection{Restart mechanism}

The final implementation detail we discuss is the brick recovery
mechanism, which is used by the failure detection mechanisms described
later.  To restart a failed brick $B_{f}$, a Dlib scans its RGID map
for the brick with the next-highest IP address $B_{r}$, and sends a
{\tt RESTART\_BRICK} message to $B_{r}$'s control channel.  If $B_{r}$
does not respond because it too has failed, the brick with the
next-highest IP address is asked to restart both bricks.  The Dlib
also removes $B_{f}$ from its RGID map so that requests are not sent
to $B_{f}$ until it recovers.

To restart the brick, $B_{r}$ runs a script that first sends a {\tt
kill -9} to $B_{f}$'s brick processes.  Next, the script attempts to
restart the brick processes.  If instead, $B_f$'s machine does not
respond at all, the node can be restarted using an IP-addressable
power source.  Since multiple Dlibs are likely to detect $B_{f}$'s
failure, $B_{r}$ does not perform recovery more than once every four
seconds (two times the beaconing interval).  Further, since restarting
a brick only cures transient failures, if the brick has been restarted
more than a threshold number of times in a given period, it is assumed
the brick has a persistent fault and should be taken offline.
Automatically reconstructing data after disk failures and allowing
failed components to be replaced en-masse, say on a weekly basis, are
next steps in our future work.


==> principles.tex <==
\section{Two principles for cheap recovery}\label{principles}

%%% * Design principles: How we achieve cheap recovery
%%%
%%%   - Tolerate replica inconsistency with quorums
%%% 
%%%     1. Quorums 101 -- read/write majority and use timestamps to
%%%        present externally consistent view
%%% 
%%%     2. Avoids data copying during recovery --> simpler, less intrusive

We follow two design principles for making recovery cheap.  The first
principle is to tolerate replica inconsistency by using quorum-based
replication~\cite{gifford:quorum}.  In the basic quorum scheme, reads
and writes are performed on a majority of the replicas.  Since the
{\em read set} and {\em write set} necessarily intersect, when we use
timestamps to compare the values returned on a read, the most
up-to-date value is returned.  Thus, quorums allow some replicas to
store stale data while the system returns up-to-date data.  What this
means in practice is that a failed replica does not need to execute
special-case recovery code to freeze writes and copy missed updates.

Although a wealth of prior work uses quorums to maintain availability
under network partitions and Byzantine failures~\cite{consist_part,
pierce:selfadjusting}\footnote{We reference two survey papers because
even a partial list of references would fill entire pages.}, few
real-life systems do this, perhaps because these failure modes are too
rare~\cite{wool:quorumload}.  Instead, we use quorums to simplify the
mechanisms for adding new nodes and rebooting failed nodes, which are
frequent occurrences in Internet services.  The main cost of
quorum-based replication is storage overhead, which we address in the
next section.

%%%   - Avoid locking/logging by using single-phase operations
%%% 
%%%     1. Avoids blocking during failure and transactional clean-up code
%%%        during recovery --> less intrusive failures, simpler recovery

The second principle is to avoid locking and transactional logging by
using single-phase operations for updates.  In replicated state stores
that use two-phase commit, recovery involves reading the log and
completing in-progress transactions by contacting other replicas.
Meanwhile, replicas holding data locks for in-progress transactions
may be forced to block until recovery is complete to reestablish full
data availability.  Using single-phase operations, we avoid locking
data during failures and cleaning up those locks on recovery.  The main
cost of single-phase operations is a weaker (but well-defined)
consistency model, which we also discuss in the next section.

%%% * Contribution: Easy-to-manage cluster-based hash table
%%% 
%%%   - Our contributions are:
%%% 
%%%     1. Identifying cheap recovery as a key to self-managing storage
%%%        systems.
%%% 
%%%     2. Design and implementation of a cluster-based hash table with
%%%        self-managing properties.

Our design principles point to two forms of coupling that exist among
replicas -- the strict consistency among replicas in ROWA and the
locking required for two-phase commit.  By removing this coupling, we
make recovery simpler and less intrusive.


==> related.tex <==
\section{Related Work}\label{related}

Motivating our work, Distributed Data Structures~\cite{gribble:dds} is
a scalable, high-performance CHT, which uses ROWA and two-phase
commit.  Session State Management~\cite{ssm-nsdi}, which shares
DStore's self-managing goals, is an in-memory CHT that provides
non-concurrent-access, semi-persistent storage for session state.
Berkeley DB~\cite{bdb}, which can serve as underlying storage for
DStore bricks, is a single-node hash table that can be replicated
using a primary-secondary scheme, but does not provide a single-system
image across a cluster.

Brick-based disk storage systems are low-cost alternatives to high-end
RAID~\cite{chen:raid} disk arrays.  Federated Array of
Bricks~\cite{frolund:hotos9} uses quorums and a non-locking two-phase
protocol to ensure linearizability.  To achieve ease of management and
performance, RepStore~\cite{zhang:repstore} uses self-organizing
capabilities of P2P DHTs and a self-tuning mechanism that replicates
frequently-written data, but trades write performance for storage by
erasure-coding read-mostly data.  In contrast to distributed disk and
file systems~\cite{petal,ganger:selfstar,zhang:repstore,frangipani}
with similar self-management goals, DStore exploits specific workload
characteristics for consistency management and exposes a higher-level
interface with guarantees on variable-sized elements.  Similarly, the
Google File System~\cite{googlefs} is designed for its large-file,
append-mostly workload to achieve scalability and manageability.

Consistency is traded for performance and
availability~\cite{brewer:giant,tact}, and
quorums~\cite{gifford:quorum} provide availability under network
partitions~\cite{consist_part} and Byzantine
faults~\cite{malkhi:phalanx,pierce:selfadjusting}; however, DStore
uses quorums and trades consistency for extremely simple persistent
state management.  Like DStore, Coda~\cite{coda} tolerates replica
inconsistency, but in a non-transparent fashion.
Bayou's~\cite{terry:bayouguarantees} {\em Monotonic Reads} and {\em
Read-Your-Writes} provide guarantees similar to those provided by
DStore's read-repair and write-in-progress cookie mechanisms; however,
Bayou's makes guarantees for a single user session, not across users.
The Porcupine Mail Server~\cite{saito:porcupine} has self-management
goals, but its {\em eventual consistency} guarantees allow users to
see data waver between old and new values before replicas eventually
become consistent.

Finally, DStore owes its statistical failure detection to
Pinpoint~\cite{chen:pinpoint}, a comprehensive, ongoing investigation
of anomaly-based failure detection.


==> roadmap.tex <==
In the rest of this paper, we discuss the principles and tradeoffs for
achieving cheap recovery (Sections
\ref{principles}-\ref{costs}); we provide implementation details
and evaluate recovery behavior (\ref{impl}-\ref{recovery-eval}); we
describe and evaluate mechanisms for failure detection and
repartitioning (\ref{failure-detect}-\ref{repartition}); and we
conclude by discussing future and related work.

